Shielded Controller Units for RL with Operational Constraints Applied to Remote Microgrids

Reinforcement learning (RL) is a powerful framework for optimizing decision-making in complex systems under uncertainty, an essential challenge in real-world settings, particularly in the context of the energy transition. A representative example is remote microgrids that supply power to communities disconnected from the main grid. Enabling the energy transition in such systems requires coordinated control of renewable sources like wind turbines, alongside fuel generators and batteries, to meet demand while minimizing fuel consumption and battery degradation under exogenous and intermittent load and wind conditions. These systems must often conform to extensive regulations and complex operational constraints. To ensure that RL agents respect these constraints, it is crucial to provide interpretable guarantees. In this paper, we introduce Shielded Controller Units (SCUs), a systematic and interpretable approach that leverages prior knowledge of system dynamics to ensure constraint satisfaction. Our shield synthesis methodology, designed for real-world deployment, decomposes the environment into a hierarchical structure where each SCU explicitly manages a subset of constraints. We demonstrate the effectiveness of SCUs on a remote microgrid optimization task with strict operational requirements. The RL agent, equipped with SCUs, achieves a 24% reduction in fuel consumption without increasing battery degradation, outperforming other baselines while satisfying all constraints. We hope SCUs contribute to the safe application of RL to the many decision-making challenges linked to the energy transition.

==> content/1_Introduction.tex <==
\section{Introduction}
\label{sec:introduction}

\hadi{Ensuring safe, sustainable, and reliable operation is critical for the control of real-world systems, especially in the context of the energy transition. These systems, such as remote microgrids serving communities without access to the main power grid,} must adhere to numerous norms and regulations. Any algorithm deployed on such a system must have its compliance to these constraints explicitly and interpretably proven. The challenge to implement robust and provable compliance guarantees for reinforcement learning (RL) agents hinders their widespread use in critical industrial settings , despite RL's potential for solving complex optimization problems in real-world  applications \citep{Dulac-Arnold2019, Kober2013}. Addressing this issue is essential for unlocking RL's full potential in industrial settings, where a wrong decision could lead to equipment damage, system failures, safety incidents, or significant economic losses \citep{Garcia2015, Amodei2016}.

White-box shielding is a promising approach to meet these requirements \citep{Alshiekh2018, Jansen2018}. Synthesized from prior knowledge of environment dynamics, a white-box shield verifies that the agent's action do not violate constraints, and imposes an alternative complying action when necessary. This mechanism, produced in human-understandable logic, can be audited by system experts, and adjusted to the desired level of conservativeness to handle the system's uncertainties. Significant progress has been made in shield synthesis \citep{Könighofer2020, Bloem_2020} and white box shielding \citep{Hsu_Hu_Fisac_2023, Krasowski_Thumm_Muller_Schafer_Wang_Althoff_2023}. However, in complex systems with many constraints across multiple devices and varying time horizons, developing a provable shield in a systematic way remains challenging. Indeed, shielding approaches usually require expressing constraints logically, simulating environment rollouts, and designing reasonably performing fallback policies. Doing so for complex environments can be tedious and error prone. A methodology decomposing the shielding problem into simpler sub-problems and allowing compliance to be proved independently for each constraint would considerably facilitate this process, enhancing the applicability of RL in critical settings.

In this paper, we propose Shielded Controllers Units (SCUs) for RL, a systematic methodology aimed at this objective. The environment is decomposed into SCUs, which link a controller to a real system to ensure the compliance of a corresponding set of constraints. Systems can be devices or a group of lower-level SCUs, forming a hierarchical structure. A controllers consists of a shielded action dispatcher and a digital twin of its corresponding system. The digital twin combines a state estimator, updated from sensor measurements, and a simulator to predict future system behavior. The shielded action dispatcher uses prior knowledge and the digital twin to test the action's validity before relaying it to the real system. Each SCU possesses a shield to guarantee compliance with its associated set of constraints. The SCU structure ensures full compliance over the whole system, while considerably simplifying the shield design process for complex real-world environment.

We demonstrate SCUs on the problem of remote microgrid optimization. Remote microgrids are small power systems disconnected from the main grid, typically powered by fossil fuel generators (\emph{gensets}). To reduce CO2 emissions and operational costs, electricity utilities are installing wind turbines for fossil-free energy. Due to the intermittent nature of wind power, large capacity batteries are needed for flexibility, while gensets remain essential to reliably meet power demand. The power dispatch problem aims to optimize the use of batteries and gensets to minimize fuel consumption and battery degradation. This complex sequential decision-making problem involves long-term planning, uncertain exogenous variables such as power demand and wind, and many constraints to ensure reliable and sustainable operation. When modeled in a realistic industrial scenario, it is a difficult problem for non-learning based optimization methods, making it an excellent use case to demonstrate the power of the shielded controllers: our RL agent outperforms baselines while its compliance to every constraint is guaranteed.
This paper makes three contributions:
\begin{itemize}
    \item It introduces Shielded Controller Units (SCUs), a systematic approach to white-box shield design, improving interpretability while ensuring constraint compliance for RL agents in industrial contexts.
    \item It presents a realistic remote microgrid optimization problem under uncertainty, aimed at training and testing an RL agent with real-world industrial considerations and constraints.
    \item The SCU approach is applied to microgrid optimization, ensuring constraint compliance while the resulting RL agent outperforms current baselines for this problem. 
    % \item Experiments provide additional insights regarding shielding RL agents, such as impact on performance and effectiveness of agent training approach.
\end{itemize}

The code for the SCU framework, the realistic microgrid environment with real wind and demand data, and the experimental process will be made available upon publication.


\iffalse
This paper is organized as follows: Section \ref{sec:related_work} reviews previous works on constrained RL, shielding, and microgrid optimization. Section \ref{sec:shielded_controller_units} presents the SCU methodology for shield design in complex systems. Section \ref{sec:remote_microgrid_optimization} describes the realistic industrial scenario of remote microgrid optimization and the application of SCU for its many constraints. Section \ref{sec:experimental_results} shows experimental results demonstrating the performance of the RL agent and additional experiments bring insights on agent shielding.
\fi

==> content/2_Related_Work.tex <==
\section{Related work}
\label{sec:related_work}

%In this section, we provide a comprehensive review of related work in the fields of constrained RL and RL for microgrid optimization. 

\hadi{
\textbf{Constrained RL} focuses on optimizing a policy while adhering to constraints and is a well-studied, ongoing area of research~\citep{wachi2024surveyconstraintformulationssafe, ijcai2021p614}. Black-box methods, such as CPO~\citep{achiam2017constrainedpolicyoptimization} and CVPO~\citep{liu2022constrainedvariationalpolicyoptimization}, use cost signals to penalize unsafe behavior but often suffer from poor interpretability and learning difficulties~\citep{mani2025risk}. Similarly, black-box shielding methods~\citep{waga2022dynamicshieldingreinforcementlearning} train classifiers to block unsafe actions but also lack transparency and struggle without environmental knowledge.
\\
In contrast, white-box shielding methods leverage known system dynamics. Early works like~\citep{bloem2012synthesis} and~\citep{Alshiekh2018} synthesized shields using formal models and constraints. More recent advances include formal verification with runtime monitoring~\citep{Fulton_Platzer_2018}, probabilistic safety constraints~\citep{Bouton_Karlsson_Nakhaei_Fujimura_Kochenderfer_Tumova_2019}, and dynamic model predictive shielding (DMPS)~\citep{Banerjee_Rahmani_Biswas_Dillig_2024}, which adapts safety interventions in real time. Reviews by~\citep{Krasowski_Thumm_Muller_Schafer_Wang_Althoff_2023} and~\citep{Hsu_Hu_Fisac_2023} highlight the promise and limitations of both black-box and model-based safety techniques. \hadi{Add factored shield reference}
\\
However, these approaches can be difficult to deploy in practice. They often require formal logic, simulated rollouts, and/or fallback policies, which are tedious and error-prone to design in complex systems. We address this by introducing a practical, modular methodology that decomposes safety enforcement into simpler shielding sub-problems—making shield design easier for each individual constraint. This improves interpretability and supports scalable, real-world application of safe RL.
Factored shield \citep{elsayed2021safe} ... }


\iffalse
\textbf{Constrained RL} is a problem where an agent must optimize a policy given a reward function while respecting constraints. It has been extensively studied and remains an active field of research~\citep{wachi2024surveyconstraintformulationssafe, ijcai2021p614}. A significant body of work focuses on black-box approaches, which assume no prior knowledge while the agent is learning. Non-shielded, cost-based methods such as CPO~\citep{achiam2017constrainedpolicyoptimization} and CVPO~\citep{liu2022constrainedvariationalpolicyoptimization} use negative costs during training to teach the agent to avoid breaking constraints. When applied to deep RL, these methods lack interpretability. Negative rewards complicate the optimization problem and can lead to challenging learning dynamics due to harder credit assignment and inadequate representation learning~\citep{mani2025risk}. Similar issues arise with black-box shielding methods~\citep{waga2022dynamicshieldingreinforcementlearning}. These methods typically train a classifier to predict if an action is safe and use it to generate a safe action as close as possible to the original action.

In both cases, black-box constrained RL methods do not include prior knowledge about the environment dynamics and consequently struggle to provide interpretable guarantees. In many industrial settings where RL is used for optimization, however, such dynamics can be modeled. This opens the door to white-box shielding, where the shield is synthesized by practitioners. This approach was used by \cite{bloem2012synthesis} and \cite{Alshiekh2018}, who designed a shield based on a formal model of the system dynamics and safety constraints. Recent studies have further explored white-box shielding. For instance, \cite{Fulton_Platzer_2018} present an approach for provably safe learning that combines formal verification with verified runtime monitoring to ensure the safety of a learning agent. \cite{Bouton_Karlsson_Nakhaei_Fujimura_Kochenderfer_Tumova_2019} propose a method to enforce probabilistic guarantees on an RL agent by constraining actions to those that satisfy a desired probabilistic specification. 
% \cite{Carr_Jansen_Junges_Topcu_2022} extend the applicability of shields to sparse-reward environments under partial observability, showing that a carefully integrated shield can improve both safety and performance in challenging environments. 
\cite{Banerjee_Rahmani_Biswas_Dillig_2024} introduce Dynamic Model Predictive Shielding (DMPS), which optimizes RL objectives while maintaining provable safety by dynamically selecting safe recovery actions. Additionally, comprehensive reviews such as \cite{Krasowski_Thumm_Muller_Schafer_Wang_Althoff_2023} provide a thorough analysis of various methods for ensuring safety in RL. Another valuable review by \cite{Hsu_Hu_Fisac_2023} emphasizes the need to combine model-based and data-driven approaches for robust safety guarantees.
However, these approaches can be difficult to deploy in practice. They often require formal logic, simulated rollouts and/or fallback policies, which are tedious and error-prone to design in complex systems. In this paper, we propose a practical, systemic methodology to decompose this into several, simpler shielding problems, allowing to simplify the shield design for every constraint. Our approach facilitates shield design and increases its interpretability, enhancing RL applicability in critical real-world settings.
\fi

\textbf{Microgrid optimization} involves managing energy sources to ensure reliable, low-emission, and sustainable operations, considering battery degradation. This complex decision-making requires long-term planning with uncertain variables like power demand and wind availability which traditional optimization techniques struggle to handle due to mixed variables and non-linear dynamics. Mixed-integer programming has had some success \citep{Hajimiragha2013, Silvente2015, Hirwa2022} but often oversimplifies constraints and overlooks battery depletion. A more realistic model by \cite{Lambert2023} allows real-time control for gensets but excludes batteries and wind turbines. Reinforcement learning (RL) approaches show promise for microgrid optimization \citep{Dimeas2010, Foruzan2018, Arwa2020, Yang2021, Wang2024} but often lack representation of industrial environments and strong safety guarantees. In \cite{Eichelbeck_Markgraf_Althoff_2022} however, RL is used for microgrid energy dispatch with similar constraints than ours, except that the dynamic constraints of fuel gensets is replaced by a constraint of robustness to islanding. Compliance is ensured by an elaborate action projection shield. Also relevant, \cite{Ceusters_Camargo_Franke_Nowé_Messagie_2023} train an RL agent for a multi-energy system and apply a safety layer verifying the compliance of constraints given an action. The compliance test can be made for a single time step based on physics equations modeling the whole system, and a simple fallback policy can be designed. Other works apply constrained RL to more general energy-related fields, such as \cite{Yu_Zhang_Song_Hui_Chen_2024} on cooling system control, \cite{Zhang_Guan_Che_Shahidehpour_2024} on electric vehicle charging, and \cite{ Chen_Shi_Arnold_Peisert_2021} on voltage regulation.


%% Previous text, which is very good too. Let's make the best of both

\iffalse

\textbf{Safe RL} The field of shield synthesis for safe reinforcement learning (RL) has evolved significantly since its inception. \cite{bloem2012synthesis} laid the theoretical groundwork for runtime enforcement through shields. This was further advanced by \cite{Alshiekh2018}, who adapted shielding to the RL context, demonstrating the use of temporal logic specifications to ensure safety during learning and deployment.

Subsequent research branched into specialized directions. Probabilistic approaches by Jansen et al. \cite{jansen2020} and \cite{hasanbeig2019} addressed stochastic systems and uncertainty. \cite{zhang2020} and \cite{avni2019} focused on learning-based shields that adapt and optimize performance. For industrial applications, \cite{wu2021} and \cite{chen2021} applied these concepts to real-time control and large-scale systems, tackling practical challenges in continuous spaces.

In the multi-agent domain, \cite{elbalghiti2022} and \cite{bouton2020} developed distributed shield architectures combined with barrier functions. Computational efficiency was a key focus for \cite{ga2021} and \cite{bharadwaj2019}, who developed fast synthesis methods for real-time systems. The challenge of scalability was addressed through compositional approaches by \cite{phan2019} and \cite{li2020}, introducing modular and hierarchical shield designs.

\textbf{Digital twin} The integration of digital twins with reinforcement learning has shown promising results across various industrial applications. \cite{chang2022digital} demonstrated the effectiveness of combining digital twins with deep reinforcement learning for real-time scheduling in flexible shop floors, showing significant improvements in production efficiency for complex products. In the autonomous driving domain, \cite{liu2021digital} proposed an end-to-end framework that leverages digital twins to train reinforcement learning agents, highlighting the importance of simulation fidelity in transferring learned policies to real-world scenarios. The application of digital twin-driven reinforcement learning extends to robotic systems, where research has shown its effectiveness in obstacle avoidance for robot manipulators through self-improving online training frameworks. \cite{xia2021digital} expanded this concept to smart manufacturing plants, developing a comprehensive framework that addresses the critical aspects of environment modeling, interface design, and intelligence integration for training deep reinforcement learning agents using digital twins.

\fi

% Another piece of text where we explain in details what we do to have a realistic representation of the industrial problem.
\iffalse
Reinforcement learning (RL) approaches have shown promising results in similar setting settings \citep{Dimeas2010, Foruzan2018, Arwa2020, Yang2021, Wang2024}, effectively showing that RL can be a solution to the problem's difficult mathematical characteristics. However, these studies often fall short in representing industrial environments in a realistic way, such that the trained RL agent could be considered for deployment in an industrial setting. In our work, the agent controls at 1 minute time steps to consider the fast dynamics of wind and demand as well as the dynamic operational constraints of devices such as gensets. Real data is used for demand and available wind power, and the predicted values the agent has access to are produced from industrially used approaches. A cycle-based battery degradation model is used, which is more realistic than often-used linear approximation. Finally, and perhaps most importantly, it includes as constraints the industrial standards that any control solution, RL or not, must comply with in order to be deployed, regarding performance, maintenance and safety. These considerably complexify the problem at hand.
\fi

==> content/3_ShieldedControllerUnits.tex <==
\section{Shielded controller units}
\label{sec:shielded_controller_units}

In complex, critical environments like real-world industrial problems, numerous constraints must be respected across systems with multiple devices. Some constraints pertain to individual devices, while other concern groups of devices, binding their control together. Ensuring compliance with a constraint sometimes requires considering future environment states to guarantee that an action is recoverable. To satisfy industrial norms, any agent deployed on such complex system must interpretably ensure compliance with these constraints, despite uncertainties from exogenous variables.
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figs/SCU_Image.png}
%     \caption{Example of SCU hierarchy. Shapes represent devices in a complex environment.}        
%     \label{fig:SCU_Example}
% \end{figure}

\begin{figure*}[!h]
    \centering
    \begin{subfigure}{0.27\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{figs/SCU_Image.png}
        \caption{Example of SCU hierarchy. Shapes represent devices in a complex environment.}
        \label{fig:SCU_Example}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.7\textwidth}
        \centering
        \includegraphics[width=0.48\linewidth]{figs/SCU-0.jpg}
        \includegraphics[width=0.48\linewidth]{figs/SCU-n.jpg}
        \caption{General SCU structure. Left: SCU for a single device. Right: higher-level SCU for a composite system.}
        \label{fig:shieldedcontrollerunit}
    \end{subfigure}
    \caption{Illustrations of Shielded Controller Units (SCUs) at different levels of abstraction.}
    \label{fig:combined_scu}
    \vspace{-5mm}
\end{figure*}

Our proposed methodology addresses this problem systematically by decomposing the environment into Shielded Controller Units (SCUs). This decomposition is based on analyzing the set of constraints. Every constraint pertains to a subset of the environment's devices, and constraints corresponding to the same subset are implemented in the same SCU. SCUs are implemented hierarchically, meaning they cannot overlap without one containing the other. For example, consider a system composed of square, triangle and star devices as shown in Figure \ref{fig:SCU_Example}. Each devices has its own constraints, and thus its own SCU: 1, 2 and 3. Two additional constraints might concern the triangle and the star: they would be managed by SCU 4. If another constraint links the triangle and square devices, whether or not the star is involved, it cannot be treated outside of SCU 4. Therefore, SCU 5 will contain both SCU 1 and SCU 4. 



\subsection{Elements of shielded controller units}

An SCU links a shielded controller to a real system. The controller's role is to receive an action from a higher-level SCU, to ensure it respects the constraints at its level, and to relay it to the real system. It contains two elements: a digital twin and a shielded dispatcher. 
The shielded dispatcher ensures compliance with constraints. It issues a compliant action for each subcomponents of the system by verifying the received actions comply with the constraints and otherwise output a complying action. Many approaches exist for white-box shielding and adequate choices must be made based on the constraint type and amount of prior knowledge. Some methods rely on state estimation \citep{Carr_Jansen_Junges_Topcu_2022} or model predictive shielding \citep{bastani2020safereinforcementlearningnonlinear, Banerjee_Rahmani_Biswas_Dillig_2024}. This need is fulfilled by the digital twin, which combines a state estimator updating its internal state based on sensor measurements, and a simulator that predicts the system's behavior given the current state and a sequence of actions. 
Importantly, the digital twin of a system must simulate the whole SCUs of its components to account for compliance of their respective constraints. This includes both a digital twin for the real system \textit{and} the digital twin inside the SCU controller, as illustrated in Figure~\ref{fig:shieldedcontrollerunit}.


% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.49\textwidth}
%     \includegraphics[width=1.0\linewidth]{figs/SCU-0.jpg}
%     % \caption{Sys 0}        
%     \label{fig:sys_0}
%     \end{subfigure}
%     \begin{subfigure}{0.49\textwidth}
%     \includegraphics[width=1.0\linewidth]{figs/SCU-n.jpg}
%     % \caption{Sys n}
%     \label{fig:sys_n}
%     \end{subfigure}
%     \caption{General structure of SCUs. On the left, an SCU applied to a single device. On the right, a higher-level SCU applied to a system with subcomponents.}
%     \label{fig:shieldedcontrollerunit}
%     \vspace{-5mm}

% \end{figure}

\subsection{Step function and interactions}

The SCU structure operates hierarchically, processing the action sent by the agent from the top level SCU down to the lower levels, and propagating the information from the devices sensors back up to the agent while updating the various levels of digital twins. This process can be realized with a single step function called from the top SCU, as described in algorithm \ref{alg:scu_step}. It is divided in three substeps.
\begin{enumerate}
    \item First, at line 3, the shield dispatcher receives action $a_t$ from the higher level and dispatches it in complying actions $\{a^{i,\mathrm{comp}}_t\}_{i = 1\dots k}$ for the $k$ sub-components $i$ using function $\textsc{Shield}$. This function is to be designed ad-hoc using an adequate interpretable shielding method, potentially using digital twin $U^{\mathrm{DT}}$
    \item Next, lines 4 to 11, the safe actions are propagated to the real system's \textsc{Step} function. If it is a device, it returns observation $o_{t+1}$. If it is a system of SCUs, it will return set $\{\hat{s}^i_{t+1}\}_{i=1\dots k}$ of state estimations of the subcomponents' SCUs. These are aggregated in observation $o_{t+1}$.
    \item Finally, at line 12, the controller internal state $s^\mathrm{SC}_{t+1}$ and its numerical twin's  $s^\mathrm{SC\cdot DT}_{t+1}$ are updated using function \textsc{UpdateController} in algorithm \ref{alg:controller_update}. $s^\mathrm{SC}_{t+1}$ is updated with ad-hoc function \textsc{ControllerState} and $s^\mathrm{SC\cdot DT}_{t+1}$ with function \textsc{UpdateDT}. If the SCU is of a device, \textsc{UpdateDT} estimates $s^\mathrm{DT}_{t+1}$ using ad-hoc estimation function \textsc{StateEstim}. If however the SCU has $k$ SCUs as sub-components $U^j$, there are 2 elements to update per $U^j$: (1) digital twin $U^{j, \mathrm{DT}}$ of the real device and (2) controller $U^{j, \mathrm{SC}}$ and its internal digital twin $U^{j, \mathrm{SC\cdot DT}}$. This implies a new recursive function propagating $o_{t+1}$ to lower levels $j$. It is disaggregated into $o^j_{t+1}$ which are used for \textsc{UpdateDT} on $U^{j, \mathrm{DT}}$ and \textsc{UpdateController} on $U^{j, \mathrm{SC}}$. Finally, the digital twin new state $s^\mathrm{DT}_{t+1}$ is the aggrefation of lower level SCU states $s^j_{t+1}$.
    

\end{enumerate}


\input{AnonymousSubmission/LaTeX/Contents_planned_main/Algorithms.tex}


\subsection{Integration within the RL framework}
The RL agent interacts with the environment using the usual Markov Decision Process (MDP) framework, but only through the highest level SCUs' step functions. These receive their respective parts of the action space's inputs and propagate them to their subcomponents down to the devices. The agent's observation is the aggregation of high-level SCUs' controllers' state estimation.




==> content/4_RemoteMicrogridOptimization.tex <==

\section{Shielded remote microgrid optimization}
\label{sec:remote_microgrid_optimization}

We consider a remote microgrid composed of a wind turbine, a battery and two fuel gensets, generating electric power to meet the demand of a village. The objective of the power dispatch problem is to control these four devices to minimize genset fuel consumption and battery depreciation, while ensuring that the generated power satisfies the demand at every time step. In this problem, two variables are considered exogenous and beyond the agent's control: demand and available wind power. Specialized industry models can provide predictions to the agent, but they are uncertain.
This problem, when realistically modeled to target industrial deployment, is an excellent test case for the SCU approach. It is of reasonable scale for in-depth analysis but complex enough that non-learning based methods struggle with real time control. RL is a powerful alternative, but it must provably respect the industrial constraints. 
In this section, we describe how we modeled the environment's physical dynamics, rewards and constraints. We also discuss how the environment is decomposed in SCUs (See Figure~\ref{fig:microgrid_scu}), the shielding approach for each controller, and define the MDP the RL agent actually interacts with.

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\linewidth]{AnonymousSubmission/LaTeX/figs/microgrid_SCU_1col.png}    
    \caption{\em SCU decomposition of the microgrid.}
\label{fig:microgrid_scu}
\vspace{-5mm}
\end{figure}

%Reinforcement learning (RL) approaches have shown promising results in similar setting settings \citep{Dimeas2010, Foruzan2018, Arwa2020, Yang2021, Wang2024}, effectively showing that RL can be a solution to the problem's difficult mathematical characteristics. However, these studies often fall short in representing industrial environments in a realistic way, such that the trained RL agent could be considered for deployment in an industrial setting. In our work, the agent controls at 1 minute time steps to consider the fast dynamics of wind and demand as well as the dynamic operational constraints of devices such as gensets. Real data is used for demand and available wind power, and the predicted values the agent has access to are produced from industrially used approaches. A cycle-based battery degradation model is used, which is more realistic than often-used linear approximation. Finally, and perhaps most importantly, it includes as constraints the industrial standards that any control solution, RL or not, must comply with in order to be deployed, regarding performance, maintenance and safety. These considerably complexify the problem at hand.

%\subsection{Simulating the microgrid}

\subsection{Exogenous variables}
There are two exogenous variables in the environment, over which the agent has no control: the power demand $\delta_t$ and the available wind power $p^\mathrm{wind, avail}_t$. We use real data gathered from remote microgrids over one year. 
Demand ranges from 180 to 540 kW, averaging 320 kW, while available wind power ranges from 0 to 400 kW, averaging 272 kW. 
The agent observes both variables at every time step and receives realistic predictions over a 30-point forecast at 15 minutes intervals, covering 7.5 hours. These predictions were generated using industry-standard approaches. Demand forecasts were produced using a general additive model (GAM) that combines transformations of the consumption observed the previous day and the previous week, along with observed and forecast temperatures \citep{demand-forecast}. 
\hadi{Wind power forecasts were generated by downscaling meteorological variables and converting them using an 8-direction power curve model. Forecasts were then fine-tuned using turbine-specific loss models, availability, and a statistical auto-adaptive model with real-time data.}
% Wind power forecasts were generated by dynamically scaling meteorological variables such as wind speed, wind direction and temperature using historical data and advanced statistical downscaling models. These variables were then transformed into available wind power using an 8-direction power curve model. Production loss models specific to the turbine, as well as wind turbine availability, were then applied to fine-tune the forecast. Finally, the forecasts were adjusted by a statistical auto-adaptive model using real-time data from the wind turbine. 

%\paragraph{Demand} Power demand from consumer's loads is an exogenous variable beyond the agent's control. We use a full year of minute-by-minute true demand data from a remote microgrid. The agent observes current demand, and 30-point forecast at 15 minutes inverval for the next 7.5 hours. Demand forecasts are generated using a general additive model (GAM) which combines transformations of the consumption observed the previous day and the previous week, as well as the observed and forecast temperature \citep{demand-forecast}. This approach is commonly used in industry for short term demand prediction, making the environment close to a real operational settings.


%\paragraph{Wind turbine} 
%The wind turbine generates renewable electric power for the microgrid by harnessing wind energy. The available wind power, an exogenous variable, is observed by the agent. The wind power produced by the turbine can be curtailed between 0 and the available wind power, without penalty. The agent also observes predictions of available wind power, as series of 30 points at 15 minutes intervals for the next 7.5 hours.
%We use true available power data from a real wind turbine, which include actual maintenance down times, as well as the associated predictions made by industrial forecast models. These predictions were generated approximately every 15 minutes for the next 24 hours. Meteorological variables such as wind speed, wind direction and temperature, from numerical weather models, were dynamically scaled using historical data and advanced statistical downscaling models. These variables were then transformed into power production using an 8-direction power curve model. Production loss models specific to the turbine were then applied, together with wind turbine availability to fine-tune the forecast. Finally, the production forecasts were adjusted by a statistical auto-adaptive model using real-time data from the wind turbine. 

\subsection{Devices}
The modeled microgrid includes three types of device: one wind turbine, two gensets, and one battery. Each device is managed by an SCU. The industrial norms they must comply with are described in \textbf{bold}. In this experiment, the digital twin sensor update function for devices and systems has been implemented as exact state update, which is realistic given the availability of precise sensors to measure relevant state variables for batteries, gensets and wind turbines.

\paragraph{Wind turbine}
The wind turbine generates renewable electric power for the microgrid by harnessing wind energy at no cost. At step $t$, it receives action $a_t = \Bar{p}^{\mathrm{wind}}_t$ containing the wind power curtailment setpoint. The resulting power $p^{\mathrm{wind}}_t$ is $\Bar{p}^{\mathrm{wind}}_t$ clipped between 0 and current available wind power $p^\mathrm{wind, avail}_t$. In this power dispatch problem, \textbf{no operational constraints applies} on the wind turbine, so the shield directly relays $a^{\mathrm{comp}}_t = a_t$ to the device.

\paragraph{Battery}
The battery stores chemical energy and can absorb or release electrical power $p^{\mathrm{batt}}_t$. The power $p^{\mathrm{batt}}_t$ responds to the $\Bar{p}^{\mathrm{batt}}_t$ setpoint from action $a_t$, can be positive (discharge) or negative (charge), and is limited by the battery nominal power of 600 kW. The battery state of charge (SoC) indicates the accumulated energy as a percentage of the battery 672 kWh capacity. Charging and discharging are inefficient processes, leading to a 5\% energy loss in each direction. We model the battery's physical behavior precisely according to \cite{G-2024-49}. The battery's degradation over charging/discharging cycles $d_{b,t}$ is modeled in arbitrary units using an approximated online rainflow algorithm adapted for MDPs, inspired from \cite{Obermayr_Riess_Wilde_2021} and \cite{Kwon_Zhu_2022} and detailed in Appendix \ref{app:battery_degradation}.  To prevent damage to the battery, the \textbf{SoC is constrained between 90 and 10\% of capacity}, or 5\% as a reserve in case of emergency. The shield uses prior knowledge of the battery inner dynamics to determine the corresponding limits and accordingly clips setpoint $\Bar{p}^{\mathrm{batt}}_t$ received from $a_t$ before relaying it as $a^{\mathrm{comp}}_t$ to the real battery. 

\paragraph{Gensets}
Gensets can produce electric power from fuel energy. We model their behavior and constraints based on \cite{Lambert2023}. Gensets receive action $a_t = (\Delta^{\mathrm{gen}}_t, \Bar{p}^{\mathrm{gen}}_t)$. Gensets's running status can be \textit{on} or \textit{off}, changed by \textit{start} or \textit{stop} command $\Delta^{\mathrm{gen}}_t$. Once \textit{on}, their power production $p^{\mathrm{gen}}_t$ is controlled by setpoint $\Bar{p}^{\mathrm{gen}}_t$ ranging between 0 and maximum power of 440 kW. Fuel consumption is proportional to $p^{\mathrm{gen}}_t$ at 0.25 l/kWh, plus a constant 10 l/h when the genset is \textit{on}.

To prevent long term damage, several operational constraints must be respected. When changing status, \textbf{gensets must complete routines}, like a 3-minute warm-up producing 100 kW or a 5-minute cool-down producing 0 kW. Once on, they have \textbf{minimum runtime} of 30 minutes during which they should not be turned \textit{off}. Except during these routines, \textit{on} gensets have a \textbf{minimal power production} of 120 kW. Producing the maximum 440 kW continuously can damage the device: \textbf{it should instead be capped at its nominal capacity} of 400 kW, except in emergencies where the 40 kW overload reserve can be used. Finally, to meet ISO 8528-1 standards \citep{iso8528-1-2018}, the \textbf{average power over the last 48 hours of operation is capped} at 70\% of nominal capacity.  
The genset SCU controller ensures these constraints are respected by modifying violating $\Delta^{\mathrm{gen}}_t$ and clipping $\Bar{p}^{\mathrm{gen}}_t$ from $a_t$ before relaying them as $a^{\mathrm{comp}}_t$ to the physical genset.

\subsection{Systems}

Two sets of operational constraints for the microgrid concern specific groups of devices, leading to two additional SCUs: the genset orchestrator and the microgrid.

\paragraph{Genset orchestrator} 
The genset orchestrator manages the two gensets, its subcomponents, by dispatching action $a_t = (\Delta^{\mathrm{orch}}_t, \Bar{p}^{\mathrm{orch}}_t)$ into actions $a^{\mathrm{comp}, i}_t = (\Delta^{\mathrm{gen}, i}_t, \Bar{p}^{\mathrm{gen}, i}_t)$ complying with two operational constraints. First, genset $i$ cannot be turned \textit{on} if genset $i - 1$ is turned \textit{off}, and vice versa. This \textbf{priority order constraint} ensures compatibility with existing heuristic-based systems so they can take over if necessary, as described in \cite{G-2024-49}. The shielded dispatcher follows a state-machine logic allowing it to turn \textit{on} or \textit{off} only one specific generator at the time. This allows to dispatch $a_t$'s single status change command $\Delta^{\mathrm{orch}}_t$ to \textit{start} or \textit{stop} a generator, or keep the current configuration, which the shield defaults to if $\Delta^{\mathrm{orch}}_t$ is inapplicable. 

The other constraint is the \textbf{equal power fraction} presented in \cite{Lambert2023}: all running genset not in warmup or cooldown must run at the same percentage of their nominal powers. The orchestrator uses its digital twin to account for single genset constraints, such as the 70\% maximum average power over 48h, as it may limit both gensets together. This constraint binds all $\Bar{p}^{\mathrm{gen}, i}_t$ together: the orchestrator dispatches them in $a^{\mathrm{comp}, i}_t$ so that the total power produced by the gensets, $p^{\mathrm{orch}}_t$, is as close as possible to the orchestrator setpoint $\Bar{p}^{\mathrm{orch}}_t$ received in $a_t$.


\paragraph{Microgrid}
The microgrid is the highest level SCU. Its objective is to ensure that \textbf{the balance, i.e. the difference between power generation and demand, is kept at 0 for all time steps}. A negative balance, or shortage,  is a critical failure of the system, while a positive balance should also be avoided although it is easier to recover from. To enforce this constraint, the microgrid subcomponents are the battery SCU, the wind turbine SCU, and the genset orchestrator SCU. Each time step, the microgrid shield dispatches complying actions $a^{\mathrm{comp}, i}_t$ to its three subcomponents, as power setpoints $\Bar{p}^{\mathrm{batt}}_t$,  $\Bar{p}^{\mathrm{wind}}_t$ and $\Bar{p}^{\mathrm{orch}}_t$, and orchestrator status change $\Delta^{\mathrm{orch}}_t$. The balance constraint, and a hard-coded wind over fuel priority, reduce the degrees of liberty of the received action $a_t$ to $\Delta^{\mathrm{orch}}_t$ and  $\Bar{p}^{\mathrm{batt}}_t$.

To ensure 0 balance, shielding operates at two levels. At any given time step $t$, the subcomponents setpoints must ensure the sum of generated powers $p^{\mathrm{batt}}_t$,  $p^{\mathrm{wind}}_t$ and $p^{\mathrm{orch}}_t$ meets demand $\delta_t$. It priorizes respecting the agent's battery setpoint, then using wind before fuel. If the demand is not met due to the limits of wind and gensets, $\Bar{p}^{\mathrm{batt}}_t$ is adjusted. If all the wind power cannot be absorbed by the demand and the battery, it is curtailed. To ensure that every subcomponent constraint is accounted for, the microgrid digital twin simulates each SCU's response to given commands. 

The shield must also avoid actions leading to irrecoverable future states, characterized by the genset orchestrator's inability to provide the power to balance the demand due to a genset being in cool-down/warm-up routine. Such blockages can take a maximum of 8 minutes.
To prevent this, a \textit{recovery shield} using a predictive shielding approach is deployed \citep{bastani2020safereinforcementlearningnonlinear, Hsu_Hu_Fisac_2023}. Monitoring is done by simulating the environment with the digital twin over a 9-minute period, given a \textit{fallback} genset orchestrator policy $\{\Delta^{\mathrm{orch}}_t, \Delta^{\mathrm{orch}}_{t+1}, \dots , \Delta^{\mathrm{orch}}_{t+8}\}$ with future $\Delta^{\mathrm{orch}}_{t+\tau} =  \mathrm{Start}$ for $\tau \in 1, \dots, 8$.  There are three unknown variables when simulating the next steps: exogenous demand, available wind power, and agent battery commands. The recovery shield guarantee should hold irrespective of the precision of exogenous variable predictions, so they are not used here. Instead, two scenarios are considered: (1) The worst case scenario with reserve, where battery command is set to discharge to the maximum, and demand and wind are simulated as rising and decreasing, respectively, towards their historical high and low at their fastest historical rate of change. The genset and battery devices are simulated as able to access their emergency reserve power. (2) A constant scenario for wind and demand, but where simulated gensets and batteries are not allowed to access their reserves.
Scenario (1) ensures a strong guarantee on the 0-balance constraint, while the (2) reduces reliance on reserve. If a negative balance is detected during one of these simulations, $\Delta^{\mathrm{orch}}_t$ is considered as possibly non-compliant and is replaced by the least different recoverable option.

\subsection{Markov Decision Process for the agent}
As the microgrid SCU is at the highest level, it interfaces with the RL agent. The agent's action space is two-dimensional: a discrete value for $\Delta^{\mathrm{orch}}_t$ and a continuous value for $\Bar{p}^{\mathrm{batt}}_t$. Its observation space includes the state estimation of the microgrid subcomponents and two time series of exogenous variable predictions -- wind and demand. 
The reward is a negative cost combining the gensets fuel consumption $\mathbf{F}_{o,t}$ (in liters) and the battery degradation $d_{b,t}$ in arbitrary units: $r_t = - (\mathbf{F}_{o,t} + \alpha d_{b,t})$, where weight $\alpha$ can be adjusted based on the utility's objective. Between equally performing solutions in terms of cost, a controller minimizing reserve usage of batteries and gensets is preferred.


==> content/5_ExperimentalResults.tex <==
\section{Experimental results}
\label{sec:experimental_results}



\subsection{Experimental setup}


We used the Soft-Actor Critic (SAC) RL algorithm \citep{haarnoja18}, which is known for its robust performance in continuous domains, to train our agents. Although we also trained the RL agents using PPO \citep{schulman2017proximalpolicyoptimizationalgorithms}, we found that SAC consistently outperformed PPO in this setting. Therefore, we report the results for the SAC agents. To process the available wind power and demand prediction time series, the agent's architecture integrates LSTMs. Details about the agent's architecture can be found in appendix \ref{app:agent_architecture}. The agents were trained on $10^5$ one-minute environment steps divided in one-day episodes. The episodes initialization involved sampling a random time during the year and the gensets and battery initial states. We explored 10 training seeds and four values of $\alpha$ for the SAC agent. Both the baselines and the trained agents were then tested in a fixed test environment consisting of the first 10 days of each month from February to November to represent varying conditions. To report the results, we averaged the performance across these 10 days. For the RL agent's performance, we also averaged the performance and calculated the standard errors across the 10 training seeds. Whenever $\alpha$ is not mentioned, it is fixed at 1.

Note that all agents use shields during evaluation unless stated otherwise. We verified that none of the constraints are violated to confirm the validity of the shield.

\begin{figure}[!h]
\vspace{-5mm}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/final_performance_plot_best_seedFalse_mean_all.png}
    \caption{\em The RL agent seeks to strike a balance between fuel consumption and battery degradation costs. Changing their respective importance in the reward function with $\alpha$ seems to exhibit the Pareto frontier. In contrast, all other baselines exhibit suboptimal performance in one or both metrics.}
    \label{fig:pareto_frontier_without_shield}
    \vspace{-5mm}

\end{figure}

% The best-performing agent for a given $\alpha$ was selected based on the average reward across these 10 days. 


\subsection{Results}

We designed our experimental section to address three research questions: (1) How do shielded RL agents perform compared to baseline algorithms in terms of minimizing fuel consumption and battery degradation? (2) How does the recovery shield impact the performance and compliance to constraints? (3) Given a shielded deployment environment, how to constrain an RL agent during training? 
% \todo{We need to write somewhere \textit{before} performance analysis that the SCU does prevent any violation for any of the constraints.}
% \begin{itemize} 
% \item How do shielded RL agents perform compared to baseline algorithms in terms of minimizing fuel consumption and battery degradation? 
% \item How does the recovery shield impact the performance and compliance to constraints? 
% \item Given a shielded deployment environment, how to incentivize and/or constrain an RL agent during training? 
% \end{itemize}


\begin{figure*}[!t]
    \centering
    % % First subfigure: smaller
    % \begin{subfigure}{0.27\linewidth}
    %     \includegraphics[width=\linewidth]{figs/final_performance_plot_best_seedFalse_mean_all.png}
    %     \caption{\em RL agents balance fuel use and battery degradation. 
    %     % The Pareto frontier is visible by varying $\alpha$, while baselines remain suboptimal.
    %     }
    %     \label{fig:pareto_frontier_without_shield}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}{0.7\linewidth}
        \includegraphics[width=\linewidth]{figs/final_plot_best_seedFalse_mean.png}
        \caption{\em Impact of the recovery shield: RL agents consume more fuel and degrade the battery more without shielding. Right: average negative balance violations ($\alpha=1$).}
        \label{fig:shielding_vs_no_shielding}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.25\linewidth}
        \includegraphics[width=\linewidth]{figs/final_shield_penalty_plot_best_seedFalse_mean_all.png}
        \caption{\em The effect of shield penalty during training. 
        % The agent trained with shielding and no penalty (blue) performs better than the one without a recoverability shield. Both the orange and green agents are more conservative due to penalties, but the orange agent has higher battery degradation, likely because learning from negative balance is easier than avoiding shields.
        }
        \label{fig:shied_usage_penalty}
    \end{subfigure}
    \caption{\em Performance of RL agents with and without recovery shielding in remote microgrid environments.}
    \label{fig:combined_rl_plots}
    \vspace{-5mm}
\end{figure*}



% \begin{figure}[bh]
%     \centering
%     \includegraphics[width=1\linewidth]{figs/final_plot_best_seedFalse_mean.png}    
%     \caption{\em Effect of the recovery shield on RL agents and baselines. (Left) RL agents exhibit increased fuel consumption and marginally higher battery degradation in the absence of recovery shield. (Right) Average negative balance violations during one day: both SAC agent and the realistic baseline avoid any negative balance with and without recovery shielding. For this plot, $\alpha=1$.}
% \label{fig:shielding_vs_no_shielding}
% % \vspace{-5mm}
% \end{figure}

\subsubsection{Performance analysis} In Figure~\ref{fig:pareto_frontier_without_shield}, we compare the performance of our RL agents with four control algorithms, detailed in supplementary materials section~\ref{sec:supp_realistic_baseline}. The \textit{random} agent performs poorly showing that relying on the SCU shield is not enough to guarantee good performance. The \textit{fuel-greedy} agent, which always attempts to turn the gensets \textit{off} and discharge the battery, consumes little fuel but highly degrades the battery. The \textit{battery-greedy} agent lets the shield change the genset status and keeps the battery idle. The battery does not degrade but fuel consumption is not optimal. The \textit{heuristic} agent reproduces a policy currently deployed in industrial settings and provides a relevant comparison point in terms of trade-off between both metrics. The RL agents trained with SAC perform significantly better, improving fuel efficiency by 9\% for similar battery degradation.  
Modifying parameter $\alpha$ to balance battery degradation cost and fuel consumption in the reward function seems to exhibit a Pareto frontier. This allows the electric utilities to trade-off battery lifetime and fuel efficiency at their preference while striking the high gain zone for remote microgrid fuel consumptions.


% \begin{figure}[tbp]
%     \centering
%     \begin{subfigure}{0.45\textwidth}
%     \includegraphics[width=0.8\linewidth]{figs/final_performance_plot_best_seedFalse_mean_all.png}
%     % \caption{Including the baselines}        
%     \label{fig:results_without_shield_reward}
%     \end{subfigure}

%     \caption{\em The RL agent seeks to strike a balance between fuel consumption and battery degradation costs. Changing their respective importance in the reward function with $\alpha$ seems to exhibit the Pareto frontier. In contrast, all other baselines exhibit suboptimal performance in one or both metrics.}
%     \label{fig:pareto_frontier_without_shield}
% % \vspace{-8mm}
% \end{figure}

\subsubsection{Impact of the recovery shield}

% \begin{figure}[bh]
%     \centering
%     \includegraphics[width=1\linewidth]{figs/final_plot_best_seedFalse_mean.png}    
%     \caption{\em Effect of the recovery shield on RL agents and baselines. (Left) RL agents exhibit increased fuel consumption and marginally higher battery degradation in the absence of recovery shield. (Right) Average negative balance violations during one day: both SAC agent and the realistic baseline avoid any negative balance with and without recovery shielding. For this plot, $\alpha=1$.}
% \label{fig:shielding_vs_no_shielding}
% % \vspace{-5mm}
% \end{figure}

In this experiment, we explore the importance of recovery shielding for both RL agents and baseline algorithms. The recovery shield is the most complex shield in this system, addressing the uncertainty of exogenous variables and requiring multi-step simulation for compliance verification. To ensure compliance in every situation, the recovery shield considers worst-case scenario which could impair performance due to over restrictiveness. Figure~\ref{fig:shielding_vs_no_shielding} presents the performance metrics and negative balance violations, with and without recovery shield. Battery-greedy agent without recovery shield has a relatively good performance but it is not acceptable due to violating the negative balance constraint. Fuel-greedy agent without recovery shield does barely consume any fuel but it also show high amount of negative balance violation. On the other hand, Heuristic policy has a stable performance even without recovery shield which shows the validity of its policy. Finally, SAC agents trained and deployed without recovery shield, but penalized for negative balance violation exhibit increased fuel consumption and slightly higher battery degradation than their shielded counterparts, while avoiding negative balance entirely (as shown in the right plot). We hypothesize that this occurs because they adopt an overly conservative and suboptimal policy due to the substantial penalties associated with negative balance during training. It is noteworthy that the RL agent with shielding shows much smaller standard errors, demonstrating the robustness of training the RL agent with a shield.

\subsubsection{How to train an RL agent given a shield?}


% \begin{figure}[!h]
% \vspace{-10mm}
%     \centering
%     \includegraphics[width=0.7\linewidth]{figs/final_shield_penalty_plot_best_seedFalse_mean_all.png}
%     \caption{\em The effect of shield penalty during training. The agent trained with shielding and no penalty (blue) performs better than the one without a recoverability shield. Both the orange and green agents are more conservative due to penalties, but the orange agent has higher battery degradation, likely because learning from negative balance is easier than avoiding shields.}
%     \label{fig:shied_usage_penalty}
% \end{figure}

A recurring research question is how penalizing the use of shielding during training impacts the agent's ability to learn an optimal policy~\citep{Hsu_Hu_Fisac_2023}. We explore this question for our use case by evaluating three variants of the RL agents with a fixed $\alpha=1$: the first agent (blue circle in Figure~\ref{fig:shied_usage_penalty}) was trained with recovery shielding but without penalizing the shield intervention. The second agent (orange) was trained with recovery shield and a penalty for shield intervention, and the third agent (green) was trained without recovery shield but with a penalty for violating the non-zero balance constraint. Note that shielding is applied to all three agents during deployment.

The agent trained with recovery shielding and no penalty (blue) achieves best performance. Both the orange and green agents learn to be more conservative due to the negative balance or shield penalty. Over-conservativeness is a known issue in punishing RL environments~\citep{mani2025risk}. Indeed, we notice these agents keep gensets \textit{on} longer which decreases the chance of receiving a penalty. Interestingly, the shield penalty seems to encourage the agent to charge the battery more probably because the shield penalty is harder to predict than the negative balance penalty for the agent.

\iffalse
These results are different from the findings of \cite{Krasowski_Thumm_Muller_Schafer_Wang_Althoff_2023}, which suggested that adding a reward penalty each time the shield intervenes improves training performance, and underlines the need for further research on the dynamics at play when training RL agents with a shield.
\fi

% This is probably expected since shielding helps with exploration of safe states and therefore, lets the RL agent learn faster. Maybe more interestingly, the same agent trained with shield but also a penalty for shield usage, achieve worse performance than the one without penalty. We believe that this happens because of the agent learn not to explore the risky yet high-reward regions of the state-space by relying to much on early shielding penalties. 



% \subsubsection{Robustness analysis}

% Another critical question for applying RL agents to real-world microgrids is how robust their performance is when there is a deviation between the model parameters and the actual system. To investigate this, we introduce noise to the parameters of the gensets and battery at both low and high levels and measure performance in terms of battery degradation and fuel consumption. We found that even ...







==> content/6_Discussion.tex <==
\section{Discussion}

While remote microgrid optimization is complex, it remains at a sufficiently small scale that it can be analyzed in depth. \cite{Eichelbeck_Markgraf_Althoff_2022} have shown that, for a very similar problem, a provable, single shield can be hand-designed to respect constraints without significantly impairing the performance. However, their paper shows the challenge of designing such a shield to comply with all constraints at once.
Our approach's applicability stands out in comparison: for every SCU, the shield is simple as it only focuses on a specific set of constraints: the others are accounted for by the SCU structure. In most cases, fallback policies are evident. Handling uncertain dynamics, such as with exogenous variables for the microgrid SCU, can be managed with the necessary level of restrictiveness. In addition, SCUs allow to analyze the degrees of freedom that each constraints removes from the RL agent, and allow it to focus on these instead of outputting actions for every device. 

A potential limitation of the SCU approach is the duplication of lower-level digital twins inside higher-level digital twins. This allows higher-level shielded controllers to consider the lower-level constraints when using rolling out strategies, but could lead to an exponential number of digital twins depending on the number of SCU levels. However, in moderately complex industrial cases, the number of SCU levels can be expected to be small \citep{siyari2019emergence}, such that scaling should not be a limiting factor.
As an example, in our case here, the depth of the SCU hierarchy is $3$.


==> content/7_Conclusion.tex <==
\vspace{-3mm}
\section{Conclusion}
\label{sec:conclusion}

This paper presented Shielded Controller Units, a decomposition approach facilitating the design of white-box shields to ensure compliance for complex constrained systems controlled by RL agents. SCUs allow to design simple shields for every constraint, which are then combined in a hierarchical structure. Digital twins pertaining to each SCU are updated at every time step so that higher-level units shields can rollout simulations accounting for lower-level constraints. 
SCUs were applied on a realistic remote microgrid optimization problem, ensuring an RL agent complying with every operational constraints. Every shield level was simple to design, describe and interpret, showcasing the applicability of SCU for provable RL compliance in complex real-world settings. 

By facilitating deployment of RL to critical systems requiring interpretable guarantees, SCUs can allow us to benefit from the potential of RL for optimizing decision-making with important social impact. We demonstrated this by showing how RL agents when supported by SCUs can reduce fuel consumption by 9\% for similar battery degradation compared to industry heuristics. We hope SCUs can be valuable for RL deployment in other regulated systems in the fields of energy, healthcare, transportation, etc.

% The SCU framework aims at being agnostic to white-box shielding methods, state estimation and simulation choices. 
% \hadi{The SCU framework is designed to be agnostic to shielding methods, state estimation, and simulation choices.} In this paper, it was demonstrated using exact sensor updates and simulation, and with logical and model predictive shielding approaches, leading to hard constraints. \hadi{When environment knowledge is partial, probabilistic shields and Bayesian estimators are more common. Future work should explore how uncertainty propagates through the SCU hierarchy.}

% When prior knowledge of the environment dynamics is partial, it is instead common to deploy probabilistic shields and Bayesian state estimation algorithms. Future works should regard resulting the propagation of uncertainty estimations through the hierarchical SCU structure.

==> content/SP1_EnvironmentDetails.tex <==


\section{Battery Degradation}\label{app:battery_degradation}

Different factors can degrade a battery and reduce its storage capacity. Time and temperature affect its capacity, however, these are not under the agent's control. More relevant here, cycling, i.e. repeated charging and discharging, significantly impacts  the battery's degradation \citep{Cao_2020}. Cycle-based battery degradation is often estimated through the rainflow analysis of the battery's state of charge  (SoC) \citep{Xu_Oudalov_Ulbig_Andersson_Kirschen_2018}, which accounts for the number and amplitude of cycles along time. However, this process is usually done offline, given a history of data. In RL however, a degradation cost $d_{b,t}$ at every time step is needed that reflects the impact of the agent's action while, when summed over a trajectory, being equal to the result of the offline process.

A commonly used approach for online battery degradation estimation is to use a linear approximation, as presented by \cite{Cao_2020}.  The linearized degradation cost is calculated using a simplified linear model, where the cost is directly proportional to the absolute value of the battery SoC change, $\text{b}_t = \text{soc}_{t} - \text{soc}_{t-1}$. The linearized degradation cost is thus computed as $d_{b,t} = \alpha_d \cdot |\text{b}_t| $ where $\alpha_d$ is the degradation coefficient. This linear approach provides a straightforward estimation of the degradation cost, making it easier to implement and understand while still capturing the essential impact of battery usage on its lifespan.  

In this paper, we aimed at representing the industrial environment as precisely as possible, and as such, to model the battery degradation more accurately. \cite{Kwon_Zhu_2022} have proposed an approach to online cycle-based degradation cost estimation for RL. In battery fatigue modeling, the impact of a cycle on degradation is exponential to the cycle amplitude. An interesting insight from \cite{Kwon_Zhu_2022} is their decomposition of the cost for each time step as
$$ d_{b,t} = \alpha_d \cdot \exp(\beta \cdot |\text{soc}_t + b_t - R[-1]|) - \alpha_d \cdot \exp(\beta \cdot |\text{soc}_t - R[-1]|)$$

where $\alpha_d$ represents the degradation rate, $\beta$ indicates the sensitivity to SoC changes, and $ R[-1] $ is the most recent switching point in the SoC history. 

The difficulty of the rainflow algorithm is however to find the right value of $R[-1]$, as cycles can close, and at the next time step, the SoC evolution can pertain to another cycle open further in history. An important problem is that, in theory, the necessary memory to correctly assign each time step to the correct value of $R[-1]$ can be as long as the complete SoC history. \cite{Kwon_Zhu_2022} propose an algorithm to keep only three points, however, it does not fully respect rainflow analysis. Instead, we based our approach on \cite{Obermayr_Riess_Wilde_2021}, where a 4-point online rainflow algorithm allows to identify the last switching point while memory requirement is hard-capped thanks to a discretization process. 
Our slightly adapted algorithm is summarized in Algorithms \ref{alg:Rainflow4P} and \ref{alg:HysteresisFilter}. The resulting buffer $R$ is used to compute the reward, and is given as an observation to the agent as part of the battery state to respect the Markovian assumption for the environment.

Note that the discretization can cause artifacts, such as the calculated degradation cost $d_{b,t}$ being negative close to switching points. In this case, we instead approximate it for this time step based on the discretization window $w$: $d_{b,t} = \alpha_d \cdot (\exp(\beta \cdot |w|) - 1) / w$.

A final question regards the value of $\alpha_d$ and $\beta$, so that $d_{b,t}$ represents a realistic capacity loss for the battery. We chose $\beta = 1$ and $\alpha_d = 5$ as in \citep{Cao_2020}. However, these values should be calibrated with a real battery if to be deployed in the real world. This explains our choice to describe the battery degradation units are arbitrary in the paper, and keep the reward function flexible with different values of weight $\alpha$.

This approach ensures that the degradation cost accurately reflects the impact of battery usage on its lifespan, considering both the magnitude and frequency of usage changes. 

\begin{minipage}{0.55\textwidth}
\begin{algorithm}[H]
\caption{Rainflow 4-point algorithm}\label{alg:Rainflow4P}
\begin{algorithmic}
\State \textcolor[rgb]{0.0, 0.5, 0.0}{\textit{// 4-point rainflow condition check}}
\Function{Rainflow4P}{R}
    \State $cycleFound \gets False$
    \If{$\min(R[-4], R[-1]) \leq \min(R[-3], R[-2])$ \textbf{and} $\max(R[-3], R[-2]) \leq \max(R[-4], R[-1])$}
        \State $cycleFound \gets True$
    \EndIf
    \State \Return $cycleFound$
\EndFunction

\State \textcolor[rgb]{0.0, 0.5, 0.0}{\textit{// Main function to update switching point buffer R}}
\Function{UpdateSwitchingPoints}{x, F, R}
    \State $F[2] \gets \textbf{Discretize}(x, d\_load)$
    \State $F, tpFound \gets \textbf{HysteresisFilter}(F)$
    \If{$tpFound$}
        \State \textbf{Append}(R, \textbf{Discretize}(F[0], d\_load))
    \EndIf
    \State \textbf{Append}(R, \textbf{Discretize}(x, d\_load))

    \While{$\textbf{Length}(R) \geq 4$ \textbf{and} \textbf{Rainflow4P}(R)}
        \State $R[-3] \gets R[-1]$
        \State \textbf{Delete}(R[-2:])
    \EndWhile
    \State \textbf{Delete}(R[-1])
    \State \Return $F, R$
\EndFunction

\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.43\textwidth}
\begin{algorithm}[H]
\caption{Hysteresis Filter algorithm}\label{alg:HysteresisFilter}
\begin{algorithmic}

\Function{HysteresisFilter}{F}
    \State \textcolor[rgb]{0.0, 0.5, 0.0}{\textit{// Apply hysteresis filter to the input signal}}
    \State \textcolor[rgb]{0.0, 0.5, 0.0}{\textit{// Define helper functions}}
    \Function{Shift}{F}
        \State $F[0] \gets F[1]$
        \State $F[1] \gets F[2]$
        \State \Return $F$
    \EndFunction
    \Function{Skip}{F}
        \State $F[1] \gets F[2]$
        \State \Return $F$
    \EndFunction

    \State $tpFound \gets False$
    \If{$F[2] < F[1]$}
        \If{$F[0] \geq F[1]$}
            \State $F \gets \textbf{Skip}(F)$
        \Else
            \State $tpFound \gets True$
            \State $F \gets \textbf{Shift}(F)$
        \EndIf
    \ElsIf{$F[2] > F[1]$}
        \If{$F[0] \leq F[1]$}
            \State $F \gets \textbf{Skip}(F)$
        \Else
            \State $tpFound \gets True$
            \State $F \gets \textbf{Shift}(F)$
        \EndIf
    \Else
        \If{$F[0] > F[1]$}
            \State $F[1] \gets \min(F[1], F[2])$
        \Else
            \State $F[1] \gets \max(F[1], F[2])$
        \EndIf
    \EndIf
    \State \Return $F, tpFound$
\EndFunction

\end{algorithmic}
\end{algorithm}
\end{minipage}


\newpage


\section{Baselines}\label{sec:supp_realistic_baseline}

The baselines are agents providing action $a_t = (\Delta^{\mathrm{orch}}_t, \Bar{p}^{\mathrm{batt}}_t)$ based on predetermined policies. 
The \textit{fuel greedy} agent sets $\Delta^{\mathrm{orch}}_t$ to \textit{stop}, and  $\Bar{p}^{\mathrm{batt}}_t$ to maximum discharging power. 
The \textit{battery greedy} agent sets $\Delta^{\mathrm{orch}}_t$ to \textit{do nothing}, and $\Bar{p}^{\mathrm{batt}}_t$ to 0.
The \textit{random} agent uniformly samples discrete $\Delta^{\mathrm{orch}}_t$ from (\textit{start, stop, do nothing}), and continuous $\Bar{p}^{\mathrm{batt}}_t$ from maximum discharging to maximum charging power.
The industry heuristics is more elaborate and reacts to the state of the microgrid. It always keeps one genset \textit{on}, and decides to turn the other genset \textit{on} when current genset is at more than 90\% of its available power (nominal or capped by the moving average constraint) for 5 minutes in a row, or directly if it reaches more than 100\%.
It turns the second genset \textit{off} if the current total genset orchestrator power coiuld be managed by 70\% of the other genset's available power for 5 minutes in a row.
On the battery side, it switches between two modes: charging, or discharging, to avoid fast cycling. In charging mode, it only charges  $\Bar{p}^{\mathrm{batt}}_t$ to capture an eventual excess power from the wind. It does not use the genset power to charge. Discharge only happens in case of emergency, as enforced by the shield. The battery charges until achieving 90\% SoC, and then switches to discharging mode. In discharging mode,  $\Bar{p}^{\mathrm{batt}}_t$ is set to maximum discharging power until the battery reaches 10\% SoC. It then switches back to charging mode.






==> content/SP2_LearningDetails.tex <==


\section{Agent architecture and learning hyper-parameters}
\label{app:agent_architecture}



\begin{figure}[bp]
    \centering
    
    \includegraphics[width=0.75\linewidth]{figs/agent_arch.png}
          
    
    \caption{The agent architecture}
    \label{fig:agent_arch}
\end{figure}

All RL agents use SAC for decision making. Both the actor and the critic use the same architecture (See Figure~\ref{fig:agent_arch}). The state is formatted as a vector and fed into a multi-layer perceptron (MLP). To take into account the predicted future demand and wind power, we added two LSTM modules which takes the demand and wind power predictions and concatenate their hidden representations with the encoded representation of the state. The final representation is passed through another MLP to compute the action probabilities and state values.

In Table~\ref{tab:learning_params}, we provide the values for the learning agent and the optimization hyper-parameters. 

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
       \multicolumn{3}{|c|}{\textbf{SAC agent}}\\
       \hline
       Observation encoder & MLP  &  2 layers (128, 32) \\       
       \hline
       Hidden dimension size & $H$ & $3\times 32$\\
       \hline
    \multicolumn{3}{|c|}{\textbf{Optimization}}\\
      \hline      
       Learning Rate & $lr$  & 0.001 or 0.0003 \\ 
      \hline
      Batch size & $B$ & 32 \\      \hline
      
    \hline
    \end{tabular}
    \caption{Learning Hyper-parameters}
    \label{tab:learning_params}
\end{table}


==> content/SP3_AdditionalResults.tex <==



\iffalse
In these section, we report ablation studies and analysis to study the role of prediction time step on the learned policy by the RL agent (Section~\ref{app:pred_timestep_section}), the effect of load/wind-power profile on the agent's behavior (Section~\ref{app:seasonal_results}), and the impact of adding a shield penalty to the objective function (Section~\ref{app:with_shield_reward}).


\subsection{The effect of prediction period} \label{app:pred_timestep_section}

The agent receives 30 exact predictions of available wind power and load for 30 points distributed over a future period $T_{pred}$, as part of its observation. We vary the timestep between these points (1, 5, and 20 minutes), to adjust the future interval the agent can access during training from 30 minutes to 10 hours. We also evaluated the agent without access to future demand and wind power predictions ($T_{pred}$ = 0). As shown in Figure~\ref{fig:pred_timestep best results}, particularly in Subfigure (a) without the shield penalty, increasing the agent’s horizon leads to better performance. This is to be expected as optimizing the decisions requires planning in the future. As such, conditioning the policy over the predictions allows the agent to achieve higher rewards. 


\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/zoomed_results_shield_0.pdf}
    \caption{The effect of prediction period ($T_{pred}$)}
    \label{fig:pred_timestep best results}
\end{figure}

% \newpage

\subsection{Adding a shield penalty }\label{app:with_shield_reward}

We tested adding a penalty for the agent when the battery power and status change in shield command $C_{M,t}$ are different from the agent action $a_t$ - meaning that the shield has modified the agent's action. Comparing Figure~\ref{fig:pareto_frontier_without_shield} and Figure~\ref{fig:pareto_frontier_with_shield}, we can observe that adding this penalty does not help the agent to converge to a better policy. This was surprising a priori, because the optimal behavior for both penalties should be the same.  Our hypothesis is that, since our agent is based on function approximation, penalizing shield usage could cause interference and affect the critic/actor function even in safe regions. Optimal policies may require actions close to the shield's threshold, which could be considered as risky by an penalized agent especially under stochastic policies such as with SAC. Developing a deeper understanding the reason behind this phenomenon and addressing it lead to interesting research questions, which we leave for future work.


\begin{figure}[tbp]
    \centering
    \begin{subfigure}{0.49\textwidth}
    \includegraphics[width=0.9\linewidth]{figs/results_shield_best_1.pdf}
    \caption{Including the baselines}        
    \label{fig:results_with_shield_reward}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
    \includegraphics[width=0.9\linewidth]{figs/zoomed_results_best_pred_1.pdf}
    \caption{Zoomed in}
    \label{fig:zoomed_results_with_shield_reward}
    \end{subfigure}
    \caption{With shield penalty}
    
    \label{fig:pareto_frontier_with_shield}
\end{figure}
\fi

==> content/ZZZZ_BatteryDegradationDraft.tex <==

\subsection{Linearized battery degradation}
The linearized degradation cost is calculated using a simplified linear model, where the cost is directly proportional to the absolute value of the battery usage, $\text{b}_t = \text{soc}_{t} - \text{soc}_{t-1}$. The formula for the linearized degradation cost is given by 
\[ \text{degradation cost} = \alpha_d \cdot |\text{b}_t| 
\] 
where \( \alpha_d \) is the degradation coefficient. This linear approach provides a straightforward estimation of the degradation cost, making it easier to implement and understand while still capturing the essential impact of battery usage on its lifespan.

\subsection{Cycle-based battery degradation}

The cycle-based degradation cost is determined by the change in SoC and the battery usage, using the formula:
\[
\text{degradation cost} = \alpha_d \cdot \exp(\beta \cdot |\text{soc}_t + b_t - R[-1]|) - \alpha_d \cdot \exp(\beta \cdot |\text{soc}_t - R[-1]|)
\]
where \( \alpha_d \) represents the degradation rate, \( \beta \) indicates the sensitivity to SoC changes, and \( R[-1] \) is the most recent switching point. If the calculated degradation cost is negative, it is normalized relative to the discretization window \( w \) using \( \text{degradation\_cost\_normalized} = \alpha_d \cdot (\exp(\beta \cdot |w|) - 1) \). The final degradation cost is then adjusted as \( \text{degradation\_cost} = |b_t| \cdot \frac{\text{degradation\_cost\_normalized}}{w} \). This approach ensures that the degradation cost accurately reflects the impact of battery usage on its lifespan, considering both the magnitude and frequency of usage changes.

\begin{minipage}{0.45\textwidth}
\begin{algorithm}[H]
\caption{Rainflow 4-point algorithm}\label{alg:Rainflow4P}
\begin{algorithmic}

\Function{Rainflow4P}{R}
    \State $cycleFound \gets False$
    \If{$\min(R[-4], R[-1]) \leq \min(R[-3], R[-2])$ \textbf{and} $\max(R[-3], R[-2]) \leq \max(R[-4], R[-1])$}
        \State $cycleFound \gets True$
    \EndIf
    \State \Return $cycleFound$
\EndFunction

\Function{UpdateSwitchingPoints}{x, F, R}
    \State $F[2] \gets \textbf{Discretize}(x, d\_load)$
    \State $F, tpFound \gets \textbf{HysteresisFilter}(F)$
    \If{$tpFound$}
        \State \textbf{Append}(R, \textbf{Discretize}(F[0], d\_load))
    \EndIf
    \State \textbf{Append}(R, \textbf{Discretize}(x, d\_load))

    \While{$\textbf{Length}(R) \geq 4$ \textbf{and} \textbf{Rainflow4P}(R)}
        \State $R[-3] \gets R[-1]$
        \State \textbf{Delete}(R[-2:])
    \EndWhile
    \State \textbf{Delete}(R[-1])
    \State \Return $F, R$
\EndFunction

\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
\begin{algorithm}[H]
\caption{Hysteresis Filter algorithm}\label{alg:HysteresisFilter}
\begin{algorithmic}

\Function{HysteresisFilter}{F}
    \State \textcolor[rgb]{0.0, 0.5, 0.0}{\textit{// Apply hysteresis filter to the input signal}}
    \State \textcolor[rgb]{0.0, 0.5, 0.0}{\textit{// Define helper functions}}
    \Function{Shift}{F}
        \State $F[0] \gets F[1]$
        \State $F[1] \gets F[2]$
        \State \Return $F$
    \EndFunction
    \Function{Skip}{F}
        \State $F[1] \gets F[2]$
        \State \Return $F$
    \EndFunction

    \State $tpFound \gets False$
    \If{$F[2] < F[1]$}
        \If{$F[0] \geq F[1]$}
            \State $F \gets \textbf{Skip}(F)$
        \Else
            \State $tpFound \gets True$
            \State $F \gets \textbf{Shift}(F)$
        \EndIf
    \ElsIf{$F[2] > F[1]$}
        \If{$F[0] \leq F[1]$}
            \State $F \gets \textbf{Skip}(F)$
        \Else
            \State $tpFound \gets True$
            \State $F \gets \textbf{Shift}(F)$
        \EndIf
    \Else
        \If{$F[0] > F[1]$}
            \State $F[1] \gets \min(F[1], F[2])$
        \Else
            \State $F[1] \gets \max(F[1], F[2])$
        \EndIf
    \EndIf
    \State \Return $F, tpFound$
\EndFunction

\end{algorithmic}
\end{algorithm}
\end{minipage}

